Seeing is Believing: Mitigating Hallucination in Large Vision-Language Models via CLIP-Guided Decoding

Large Vision-Language Models (LVLMs) are susceptible to object hallucinations, an issue in which their generated text contains non-existent objects, greatly limiting their reliability and practicality. Current approaches often rely on the model's token likelihoods or other internal information, instruction tuning on additional datasets, or incorporating complex external tools. We first perform empirical analysis on sentence-level LVLM hallucination, finding that CLIP similarity to the image acts as a stronger and more robust indicator of hallucination compared to token likelihoods. Motivated by this, we introduce our CLIP-Guided Decoding (CGD) approach, a straightforward but effective training-free approach to reduce object hallucination at decoding time. CGD uses CLIP to guide the model's decoding process by enhancing visual grounding of generated text with the image. Experiments demonstrate that CGD effectively mitigates object hallucination across multiple LVLM families while preserving the utility of text generation. Codes are available at https://github.com/d-ailin/CLIP-Guided-Decoding.

==> tables/coco.tex <==

\begin{table*}[t]
\centering
 \caption{Hallucination evaluation on COCO Caption Karpathy Test~\cite{karpathy2015deep}. For additional metrics, please refer to Table~\ref{tab:coco_full} in Appendix. \ailin{todo: update the numeric results, add DoLa result, add coverage ratio and hallucination ratios}}
 % \caption{Hallucination evaluation on MSCOCO is performed under three LVLMs using CHAIR$_S$ ($C_S$) and CHAIR$_I$ ($C_I$), where smaller values indicate less object hallucination. For additional metrics, please refer to Appendix.}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
  \ & \multicolumn{3}{c|} {InstructBLIP}  &\multicolumn{3}{c|} {mPLUG-Owl2}  & \multicolumn{3}{c} {LLaVA-1.5}       \\
  &$C_S$ $\downarrow$ & $C_I$ $\downarrow$ & \small{Avg. Len} 
  &$C_S$ $\downarrow$ & $C_I$ $\downarrow$ & \small{Avg. Len}
  &$C_S$ $\downarrow$ & $C_I$ $\downarrow$ & \small{Avg. Len}\\
   \midrule
Greedy & 60.7 & 25.8 & 108.4 &  53.6 & 15.2 & 89.9  &  46.0 & 12.9 & 81.4\\
Nucleus  &  56.1 & 17.0 & 98.3 &  51.8 & 14.8 & 90.0  &  46.6 & 13.6 & 81.1 \\
TopK &  55.8 & 16.9 & 97.3 &  54.0 & 15.3 & 89.4  &  46.6 & 13.5 & 81.0 \\
\midrule
\textbf{\ours\ (ours)} & \textbf{42.7} & \textbf{10.9} & 99.6 & \textbf{35.2} & \textbf{7.9} & 85.1 & \textbf{31.4} & \textbf{7.9} & 77.3 \\
\bottomrule
\end{tabular}
\label{tab:coco}
\end{table*}



==> tables/coco_full.tex <==

% \begin{tabular}{lllllllllllll}
\begin{table*}[h]
    \centering
    \setlength\tabcolsep{2.5pt}
    \caption{Hallucination evaluation results on COCO.}
    \label{tab:coco_full}
    \footnotesize
    \begin{tabular}{cccccccccccccccc}
    \toprule
    Model &  & 
    % Cs↓ & Ci↓ & Avg. Length↑ & \makecell{Avg.\\Object}↑ & \makecell{Avg. Hall\\ Object}↓ & BLEU-1↑ & BLEU-2↑ & BLEU-3↑ & BLEU-4↑ & METEOR↑ & ROUGE-L↑ & SPICE↑ & CLIPS↑ \\

    % Cs$\downarrow$ & Ci$\downarrow$ & Avg. Length$\uparrow$ & Avg. Object$\uparrow$ & Avg. Hallucination Object$\downarrow$ & BLEU-1$\uparrow$ & BLEU-2$\uparrow$ & BLEU-3$\uparrow$ & BLEU-4$\uparrow$ & METEOR$\uparrow$ & ROUGE-L$\uparrow$ & SPICE$\uparrow$ & CLIPS$\uparrow$ \\

    % \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\ Length\\($\uparrow$)} & \makecell{Avg. \\Object\\($\uparrow$)} & \makecell{Avg. Hallu\\ Object\\($\downarrow$)} & \makecell{BLEU-1\\($\uparrow$)} & \makecell{BLEU-2\\($\uparrow$)} & \makecell{BLEU-3\\($\uparrow$)} & \makecell{BLEU-4\\($\uparrow$)} & \makecell{METEOR\\($\uparrow$)} & \makecell{ROUGE-L\\($\uparrow$)} & \makecell{SPICE\\($\uparrow$)} & \makecell{CLIPS\\($\uparrow$)} \\

    \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\Length\\($\uparrow$)} & \makecell{Avg.\\Coverage\\($\uparrow$)} & \makecell{Avg.\\Object\\($\uparrow$)} & \makecell{Avg.\\Hallu. Object\\($\downarrow$)} & \makecell{BLEU-1\\($\uparrow$)} & \makecell{BLEU-2\\($\uparrow$)} & \makecell{BLEU-3\\($\uparrow$)} & \makecell{BLEU-4\\($\uparrow$)} & \makecell{METEOR\\($\uparrow$)} & \makecell{ROUGE-L\\($\uparrow$)} & \makecell{SPICE\\($\uparrow$)} & \makecell{CLIPS\\($\uparrow$)} \\

    


    \midrule
    \multirow{4}*{InstructBLIP}
    & Greedy & 57.93 & 17.14 & \textbf{102.65} & \textbf{81.10} & 7.53 & 1.56 & 15.85 & 10.97 & 7.02 & 4.41 & 17.12 & 16.99 & 17.69 & 27.06 \\
    & Nucleus & 56.13 & 16.95 & 98.30 & 80.61 & 7.25 & 1.48 & 16.38 & 11.29 & 7.21 & 4.53 & 17.45 & 17.46 & 18.17 & 27.05 \\
    & TopK & 55.80 & 16.88 & 97.26 & 80.04 & 7.13 & 1.45 & 16.46 & 11.26 & 7.13 & 4.43 & 17.36 & 17.48 & 18.00 & 27.03 \\
    & Ours & \textbf{42.73} & \textbf{10.85} & 99.64 & 79.44 & 7.97 & 0.97 & 16.38 & 11.30 & 7.19 & 4.50 & 17.44 & 17.49 & \textbf{18.46} & \textbf{28.24} \\

    \midrule
    \multirow{4}*{mPLUG-Owl2}
    & Greedy & 52.67 & 15.97 & \textbf{89.35} & 81.28 & 6.57 & 1.25 & 18.08 & 12.59 & 8.28 & 5.39 & 18.79 & 19.28 & 19.18 & 27.08 \\
    & Nucleus & 51.87 & 15.62 & 88.98 & 81.68 & 6.67 & 1.23 & 18.12 & 12.60 & 8.26 & 5.36 & 18.78 & 19.38 & 19.30 & 27.05 \\
    & TopK & 53.13 & 15.90 & 89.15 & 81.36 & 6.58 & 1.24 & 18.09 & 12.51 & 8.18 & 5.29 & 18.76 & 19.38 & 19.22 & 27.06 \\
    & Ours & 35.67 & 8.59 & 85.06 & 80.17 & \textbf{7.05} & 0.66 & 19.07 & 13.42 & \textbf{8.88} & \textbf{5.77} & 19.37 & 20.35 & 20.21 & 28.21 \\


    \midrule
    \multirow{5}*{LLaVA-1.5}
    & Greedy & 44.67 & 13.11 & 80.05 & 81.30 & 6.09 & 0.92 & 18.91 & 12.73 & 8.07 & 5.07 & 18.69 & 20.23 & 18.49 & 26.94 \\
    & Nucleus & 43.27 & 13.12 & 80.14 & 81.19 & 6.06 & 0.92 & 18.88 & 12.77 & 8.10 & 5.12 & 18.73 & 20.25 & 18.50 & 26.93 \\
    & TopK & 44.87 & 13.18 & 79.71 & 81.39 & 6.07 & 0.92 & 18.90 & 12.69 & 8.05 & 5.07 & 18.66 & 20.20 & 18.39 & 26.92 \\
    & DoLa & 46.60 & 13.62 & 80.29 & 80.88 & 6.06 & 0.96 & 18.74 & 12.46 & 7.83 & 4.88 & 18.55 & 19.98 & 17.98 & 26.81 \\
    & Ours & 29.73 & 8.12 & 76.66 & 79.03 & 6.36 & 0.56 & 19.85 & 13.46 & 8.60 & 5.43 & 19.34 & 21.13 & \textbf{19.37} & 27.96 \\


    \bottomrule
    \end{tabular}    
\end{table*}


==> tables/coco_hallu.tex <==

% \begin{tabular}{lllllllllllll}
\begin{table}[t]
    \centering
    % \setlength\tabcolsep{2.5pt}
    \caption{Hallucination evaluation results on COCO.}
    \label{tab:coco_hallu}
    \small
    % \begin{tabular}{crcc|c}
    \begin{tabular}{crccc}
    \toprule
    Model &  & 
    % Cs↓ & Ci↓ & Avg. Length↑ & \makecell{Avg.\\Object}↑ & \makecell{Avg. Hall\\ Object}↓ & BLEU-1↑ & BLEU-2↑ & BLEU-3↑ & BLEU-4↑ & METEOR↑ & ROUGE-L↑ & SPICE↑ & CLIPS↑ \\

    % Cs$\downarrow$ & Ci$\downarrow$ & Avg. Length$\uparrow$ & Avg. Object$\uparrow$ & Avg. Hallucination Object$\downarrow$ & BLEU-1$\uparrow$ & BLEU-2$\uparrow$ & BLEU-3$\uparrow$ & BLEU-4$\uparrow$ & METEOR$\uparrow$ & ROUGE-L$\uparrow$ & SPICE$\uparrow$ & CLIPS$\uparrow$ \\

    % \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\ Length\\($\uparrow$)} & \makecell{Avg. \\Object\\($\uparrow$)} & \makecell{Avg. Hallu\\ Object\\($\downarrow$)} & \makecell{BLEU-1\\($\uparrow$)} & \makecell{BLEU-2\\($\uparrow$)} & \makecell{BLEU-3\\($\uparrow$)} & \makecell{BLEU-4\\($\uparrow$)} & \makecell{METEOR\\($\uparrow$)} & \makecell{ROUGE-L\\($\uparrow$)} & \makecell{SPICE\\($\uparrow$)} & \makecell{CLIPS\\($\uparrow$)} \\

    \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\Length}\\

    


    \midrule
    \multirow{4}*{InstructBLIP}
    % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize{InstructBLIP}}}}
    % & Greedy & 60.70 & 25.82 & \textbf{108.37} & 3.33 & 1.16 & 14.89 & 7.36 & 4.14 & 2.38 & 13.73 & 13.18 & 13.84 & 25.30 \\
    & Greedy & 57.93 & 17.14 & 102.65 \\
    & Nucleus & 56.13 & 16.95 & 98.30 \\
    & TopK & 55.80 & 16.88 & 97.26 \\
    & DoLa & 55.60 & 17.03 & 97.11 \\
    & Ours & \textbf{42.73} & \textbf{10.85} & 99.64 \\

    \midrule
    \multirow{4}*{mPLUG-Owl2}
    & Greedy & 52.67 & 15.97 & 89.35 \\
    & Nucleus & 51.87 & 15.62 & 88.98 \\
    & TopK & 53.13 & 15.90 & 89.15\\
    & DoLa & 52.60 & 15.23 & 88.76 \\
    & Ours & \textbf{35.67} &\textbf{ 8.59} & 85.06\\


    \midrule
    \multirow{5}*{LLaVA-1.5}
    & Greedy & 44.67 & 13.11 & 80.05 \\
    & Nucleus & 43.27 & 13.12 & 80.14 \\
    & TopK & 44.87 & 13.18 & 79.71 \\
    & DoLa & 46.60 & 13.62 & 80.29 \\
    & Ours & \textbf{29.73} & \textbf{8.12} & 76.66 \\


    \bottomrule
    \end{tabular}    
\end{table}


==> tables/hyper_all.tex <==

\begin{minipage}[t]{.45\textwidth}
\footnotesize % Smaller font size for the table
\captionof{table}{\small Sensitivity and efficiency analysis of maximum candidate number N and sampling times M. Time: inference time (s) per sample.}
\label{tab:table1}
\begin{tabular}{@{}llllrr@{}} % Added @{\extracolsep{\fill}} for spacing
\toprule
Method & N & M & \(C_S \downarrow\) & \(C_I \downarrow\) & Time \\
\midrule
Greedy & - & - & 44.67 & 13.11 & 3.79 \\
VCD    & - & - & 44.60 & 12.54 & 7.31 \\
OPERA  & - & - & 49.52 & 13.70 &  \\
CGD    & 1 & 3 & 37.66 &  9.90 & 7.07 \\
       & 1 & 5 & 34.50 & 8.95 & 10.24 \\
        & 3 & 3 & 29.73 & 8.12 &  \\
        & 5 & 3 & \textbf{28.40} & \textbf{6.78} &  \\
\bottomrule
\end{tabular}
\vspace{2mm}
\centering
\footnotesize % Smaller font size for the table
\captionof{table}{\small Sensitivity analysis of CLIP-guidance model.}
\label{tab:table2}
\begin{tabular}{@{}llr@{}}
\toprule
Method & \(C_S \downarrow\) & \(C_I \uparrow\) \\
\midrule
Greedy & 44.67 & 13.11 \\
w/ SigLIP ViT-SO-14@384px & 29.73 &  8.12 \\
w/ OpenAI ViT-L-14@336px & 32.80 &  8.78 \\
\bottomrule
\end{tabular}
\end{minipage}



==> tables/hyper_alpha.tex <==

\begin{table}[h]
    \centering
    \footnotesize
    % \setlength\tabcolsep{2.5pt}
    \caption{Ablation study on scoring components in~\Cref{eq:scoring_func}.}
    \label{tab:ablation}
    \begin{tabular}{lccc}
    \toprule
    Method  & 
    % Cs↓ & Ci↓ & Avg. Length↑ & \makecell{Avg.\\Object}↑ & \makecell{Avg. Hall\\ Object}↓ & BLEU-1↑ & BLEU-2↑ & BLEU-3↑ & BLEU-4↑ & METEOR↑ & ROUGE-L↑ & SPICE↑ & CLIPS↑ \\

    % Cs$\downarrow$ & Ci$\downarrow$ & Avg. Length$\uparrow$ & Avg. Object$\uparrow$ & Avg. Hallucination Object$\downarrow$ & BLEU-1$\uparrow$ & BLEU-2$\uparrow$ & BLEU-3$\uparrow$ & BLEU-4$\uparrow$ & METEOR$\uparrow$ & ROUGE-L$\uparrow$ & SPICE$\uparrow$ & CLIPS$\uparrow$ \\

    % \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\ Length} \\
    \makecell{$C_S$ $\downarrow$} & \makecell{$C_I$ $\downarrow$} & \makecell{Avg. Len}\\
    \midrule
    Greedy & 44.67  & 13.11 & 80.05 \\
    \midrule

    \ours\ (Ours) & 29.73 & 8.12 & 76.66 \\
    w/o Sentence Likelihood  & \textbf{29.45} & \textbf{7.37} & 76.12 \\
    w/o CLIP-Guidance & 45.07 & 13.29 & 81.60 \\

    \bottomrule
    \end{tabular}    
\end{table}




==> tables/hyper_clip.tex <==
\begin{table}[h]
    \centering
    % \setlength\tabcolsep{2.5pt}
    \footnotesize
    \caption{Sensitivity analysis of CLIP-guidance model.}
    \label{tab:hyper_clip}
    \begin{tabular}{lccc}
    \toprule
    Method  & 
    % Cs↓ & Ci↓ & Avg. Length↑ & \makecell{Avg.\\Object}↑ & \makecell{Avg. Hall\\ Object}↓ & BLEU-1↑ & BLEU-2↑ & BLEU-3↑ & BLEU-4↑ & METEOR↑ & ROUGE-L↑ & SPICE↑ & CLIPS↑ \\

    % Cs$\downarrow$ & Ci$\downarrow$ & Avg. Length$\uparrow$ & Avg. Object$\uparrow$ & Avg. Hallucination Object$\downarrow$ & BLEU-1$\uparrow$ & BLEU-2$\uparrow$ & BLEU-3$\uparrow$ & BLEU-4$\uparrow$ & METEOR$\uparrow$ & ROUGE-L$\uparrow$ & SPICE$\uparrow$ & CLIPS$\uparrow$ \\

    % \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\ Length} \\
    \makecell{$C_S$ $\downarrow$} & \makecell{$C_I$ $\downarrow$} & \makecell{Avg. Len}\\
    \midrule
    Greedy &  44.67  & 13.11 & 80.05 \\
    \midrule

    w/ SigLIP ViT-SO-14@384px & \textbf{29.73} & \textbf{8.12} & 76.66 \\
    w/ OpenAI ViT-L-14@336px & 32.80 & 8.78 & 75.83 \\

    \bottomrule
    \end{tabular}    
\end{table}

==> tables/hyper_nm.tex <==

% \begin{tabular}{lllllllllllll}
\begin{table}[h]
    \centering
    % \setlength\tabcolsep{2.5pt}
    \footnotesize
    \caption{ Sensitivity and efficiency analysis of maximum candidate number $N$ and sampling times $M$. Time: inference time (s) per sample.}
    \label{tab:hyper_nm}
    \begin{tabular}{crrccc|c}
    \toprule
    Method & $N$ & $M$  & 
    % Cs↓ & Ci↓ & Avg. Length↑ & \makecell{Avg.\\Object}↑ & \makecell{Avg. Hall\\ Object}↓ & BLEU-1↑ & BLEU-2↑ & BLEU-3↑ & BLEU-4↑ & METEOR↑ & ROUGE-L↑ & SPICE↑ & CLIPS↑ \\

    % Cs$\downarrow$ & Ci$\downarrow$ & Avg. Length$\uparrow$ & Avg. Object$\uparrow$ & Avg. Hallucination Object$\downarrow$ & BLEU-1$\uparrow$ & BLEU-2$\uparrow$ & BLEU-3$\uparrow$ & BLEU-4$\uparrow$ & METEOR$\uparrow$ & ROUGE-L$\uparrow$ & SPICE$\uparrow$ & CLIPS$\uparrow$ \\

    % \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg.\\ Length}\\
    \makecell{$C_S$ $\downarrow$} & \makecell{$C_I$ $\downarrow$} & \makecell{Avg. Len} & \makecell{Time}\\
    \midrule
    Greedy & - & - & 44.67  & 13.11 & 80.05 & 3.78/6.25 \\
    VCD & - & - & 44.60 & 12.54 & 85.80 & 8.25 \\
    OPERA & - & - & 49.52 & 13.70 & 85.71 &  \\
    \midrule
    \multirow{4}*{\ours}
    & 1 & 3 & 37.66 & 9.90 & 78.67 \\
    & 1 & 5 & 34.50 & 8.95 & 78.70 \\
    & 3 & 3 & 29.73 & 8.12 & 76.66 \\
    & 5 & 3 & \textbf{28.40} & \textbf{6.78} & 78.18 \\
    \bottomrule
    \end{tabular}    
\end{table}



==> tables/hyper_nm_clip.tex <==


\noindent
\begin{minipage}[t]{.5\textwidth}
\centering
\small % Smaller font size for the table
\captionof{table}{\small Sensitivity and efficiency analysis of maximum candidate number N and sampling times M. Time: inference time (s) per sample.}
\label{tab:table1}
\begin{tabular}{@{}llllrr@{}} % Added @{\extracolsep{\fill}} for spacing
\toprule
Method & N & M & \(C_S \downarrow\) & \(C_I \downarrow\) & Time \\
\midrule
Greedy & - & - & 44.67 & 13.11 & 3.79 \\
VCD    & - & - & 44.60 & 12.54 & 7.31 \\
OPERA  & - & - & 49.52 & 13.70 & 44.33 \\
CGD    & 1 & 3 & 37.66 &  9.90 & 7.07 \\
       & 1 & 5 & 34.50 & 8.95 & 10.24 \\
        & 3 & 3 & 29.73 & 8.12 &  \\
        & 5 & 3 & \textbf{28.40} & \textbf{6.78} &  \\
\bottomrule
\end{tabular}
\end{minipage}%
\hfill
\begin{minipage}[t]{.46\textwidth}
\centering
\small % Smaller font size for the table
\captionof{table}{\small Sensitivity analysis of CLIP-guidance model.}
\label{tab:table2}
\begin{tabular}{@{}llr@{}}
\toprule
Method & \(C_S \downarrow\) & \(C_I \uparrow\) \\
\midrule
Greedy & 44.67 & 13.11 \\
w/ SigLIP ViT-SO-14@384px & 29.73 &  8.12 \\
w/ OpenAI ViT-L-14@336px & 32.80 &  8.78 \\
\bottomrule
\end{tabular}
\end{minipage}



==> tables/nocaps.tex <==


\begin{table*}[t]
\centering
 \caption{Hallucination evaluation on NoCaps (Near-Domain and Out-of-Domain)~\cite{agrawal2019nocaps}.}
 % \caption{Hallucination evaluation on Nocaps (out-domain) is performed under three LVLMs using CHAIR$_S$ ($C_S$) and CHAIR$_I$ ($C_I$), where smaller values indicate less object hallucination. For additional metrics, please refer to Appendix.}
 \footnotesize
\begin{tabular}{l|l|ccc|ccc|ccc}
\toprule
  \Dataset &  & \multicolumn{3}{c|} {InstructBLIP}  &\multicolumn{3}{c|} {mPLUG-Owl2}  & \multicolumn{3}{c} {LLaVA-1.5}       \\
  & &$C_S$ $\downarrow$ & $C_I$ $\downarrow$ & \small{Avg. Len} 
  &$C_S$ $\downarrow$ & $C_I$ $\downarrow$ & \small{Avg. Len}
  &$C_S$ $\downarrow$ & $C_I$ $\downarrow$ & \small{Avg. Len}\\
   \midrule
% Original & 26.8&7.3 & 54.0 & 11.3  &  56.6 & 11.0 & 11.3  &  56.6 & 11.0\\
\multirow{5}{*}{\shortstack{NoCaps\\(Near-Domain)}} & 
Greedy & 55.7 & 15.4 & 102.9 & 39.5 & 10.1 & 77.7  &  46.1 & 12.2 & 80.0 \\
& Nucleus  & 54.1 & 14.7 & 98.9 &  40.9 & 10.6 & 78.0 &  45.4 & 11.9 & 79.5 \\
& TopK &  53.2 & 14.1 & 98.6 & 41.6  & 10.9 & 78.1 &  46.6 & 12.1 & 79.8 \\
& DoLa & 54.5 & 14.0 & 97.9 & 41.0 & 10.8 & 77.9 & 44.8 & 12.1 & 79.5 \\
\cmidrule{2-11}
& \textbf{\ours\ (ours)} & \textbf{42.6} & \textbf{12.3} & 100.6 & \textbf{29.0} & \textbf{6.9} & 72.8 &  \textbf{33.3} & \textbf{7.9} & 75.9 \\
\midrule
\multirow{4}{*}{\shortstack{NoCaps\\(Out-of-Domain)}} & 
Greedy & 51.3 & 17.3 & 98.4 & 36.4 & 12.4 & 68.0  &  40.2 & 14.2 & 69.1\\
& Nucleus  & 48.8 & 16.3 & 92.8  & 36.8 & 12.1 & 68.8  &  40.7 & 14.3 & 69.4 \\
& TopK &  50.3 & 17.0 & 92.2 & 37.1 & 12.3 & 68.2 &  39.9 & 13.5 & 69.5 \\
& DoLa & 48.0 & 16.3 & 92.3 & 35.9 & 13.2 & 68.3 & 43.5 & 14.4 & 71.1 \\
\cmidrule{2-11}
& \textbf{\ours\ (ours)} & \textbf{42.0} & \textbf{11.6} & 94.1 & \textbf{26.6} & \textbf{8.4} & 65.7 & \textbf{28.8} & \textbf{9.0} & 66.3 \\
\bottomrule
\end{tabular}
\label{tab:nocaps}
\end{table*}


==> tables/nocaps_full.tex <==

% \begin{tabular}{lllllllllllll}
\begin{table*}[h]
    \centering
    % \setlength\tabcolsep{2.5pt}
    \caption{Hallucination evaluation results on NoCaps (Near-Domain and Out-of-Domain) with three LVLM models.}
    \label{tab:nocaps_full}
    \begin{tabular}{clccccccc}
    \toprule
    & Model &  & 
    % Cs↓ & Ci↓ & Avg. Length↑ & \makecell{Avg.\\Object}↑ & \makecell{Avg. Hall\\ Object}↓ & BLEU-1↑ & BLEU-2↑ & BLEU-3↑ & BLEU-4↑ & METEOR↑ & ROUGE-L↑ & SPICE↑ & CLIPS↑ \\

    % Cs$\downarrow$ & Ci$\downarrow$ & Avg. Length$\uparrow$ & Avg. Object$\uparrow$ & Avg. Hallucination Object$\downarrow$ & BLEU-1$\uparrow$ & BLEU-2$\uparrow$ & BLEU-3$\uparrow$ & BLEU-4$\uparrow$ & METEOR$\uparrow$ & ROUGE-L$\uparrow$ & SPICE$\uparrow$ & CLIPS$\uparrow$ \\

    \makecell{$C_S$\\($\downarrow$)} & \makecell{$C_I$\\($\downarrow$)} & \makecell{Avg. Length\\($\uparrow$)} & \makecell{Avg. Object\\($\uparrow$)} & \makecell{Avg. Hallu Object\\($\downarrow$)} & \makecell{CLIPS\\($\uparrow$)} \\

    \midrule
    \multirow{12}*{Near-Domain}
    & \multirow{4}*{InstructBLIP} 
    & Greedy & 60.20 & 21.28 & \textbf{110.22} & 4.29 & 1.16 & 25.40 \\
    & & Nucleus & 54.07 & 14.65 & 98.92 & 7.79 & 1.34 & 26.41 \\
    & & TopK & 53.20 & 14.14 & 98.62 & 7.77 & 1.28 & 26.47 \\
    & & Ours & \textbf{44.60} & \textbf{9.90} & 100.56 & \textbf{8.10} & \textbf{0.89} & \textbf{27.79} \\

    \cmidrule{2-9}
    & \multirow{4}*{mPLUG-Owl2} 
    & Greedy & 39.53 & 10.07 & 77.70 & \textbf{6.63} & 0.74 & 26.61 \\
    & & Nucleus & 40.93 & 10.59 & 77.95 & 6.62 & 0.78 & 26.60 \\
    & & TopK & 41.60 & 10.85 & \textbf{78.14} & 6.57 & 0.80 & 26.54 \\
    & & Ours & \textbf{29.00} & \textbf{6.85} & 72.76 & 6.47 & \textbf{0.48 }& \textbf{27.76} \\
    

    \cmidrule{2-9}
    & \multirow{4}*{LLaVA-1.5}
    & Greedy & 46.13 & 12.19 & \textbf{79.99} & 6.41 & 0.89 & 26.23 \\
    & & Nucleus & 45.40 & 11.92 & 79.54 & 6.38 & 0.86 & 26.21 \\
    & & TopK & 46.60 & 12.07 & 79.80 & 6.32 & 0.87 & 26.18 \\
    & & Ours & \textbf{33.27} & \textbf{7.86} & 75.86 & \textbf{6.46} & \textbf{0.55} & \textbf{27.36} \\
    \midrule

    \multirow{12}*{Out-of-Domain}
    & \multirow{4}*{InstructBLIP} 
    & Greedy & 59.67 & 24.51 & \textbf{104.20} & 3.68 & 1.19 & 25.92 \\
    & & Nucleus & 48.80 & 16.28 & 92.76 & 6.68 & 1.30 & 27.68 \\
    & & TopK & 50.33 & 17.02 & 92.21 & 6.59 & 1.35 & 27.64 \\
    & & Ours & \textbf{42.00} & \textbf{11.62} & 94.11 & \textbf{7.09} & \textbf{0.93} & \textbf{28.90} \\


    \cmidrule{2-9}
    & \multirow{4}*{mPLUG-Owl2} 
    & Greedy & 36.40 & 12.35 & 67.95 & 5.15 & 0.73 & 27.85 \\
    & & Nucleus & 36.80 & 12.13 & \textbf{68.83} & \textbf{5.26} & 0.73 & 27.84 \\
    & & TopK & 37.13 & 12.27 & 68.17 & 5.13 & 0.72 & 27.80 \\
    & & Ours & \textbf{26.60} & \textbf{8.38} & 65.67 & 5.14 & \textbf{0.47} & \textbf{28.73} \\

    

    \cmidrule{2-9}
    & \multirow{4}*{LLaVA-1.5}
    & Greedy & 40.20 & 14.21 & 69.07 & 5.13 & 0.85 & 27.48 \\
    & & Nucleus & 40.67 & 14.26 & 69.39 & 5.12 & 0.85 & 27.48 \\
    & & TopK & 39.87 & 13.51 & \textbf{69.54} & 5.17 & 0.81 & 27.51 \\
    & & Ours & \textbf{28.80} & \textbf{8.99} & 66.34 & \textbf{5.21} & \textbf{0.51} & \textbf{28.45} \\

    
    \bottomrule
    \end{tabular}    
\end{table*}

